Provable Privacy with Non-Private Pre-Processing

When analysing Differentially Private (DP) machine learning pipelines, the potential privacy cost of data-dependent pre-processing is frequently overlooked in privacy accounting. In this work, we propose a general framework to evaluate the additional privacy cost incurred by non-private data-dependent pre-processing algorithms. Our framework establishes upper bounds on the overall privacy guarantees by utilising two new technical notions: a variant of DP termed Smooth DP and the bounded sensitivity of the pre-processing algorithms. In addition to the generic framework, we provide explicit overall privacy guarantees for multiple data-dependent pre-processing algorithms, such as data imputation, quantization, deduplication and PCA, when used in combination with several DP algorithms. Notably, this framework is also simple to implement, allowing direct integration into existing DP pipelines.

==> main_files/low-dimensional-OLS.tex <==
1

Let $\algprivols$ be the private low-dimensional OLS estimator projected by the matrix $D$ with Guassian noise. Given a dataset $(X, Y)\in \reals^{n\times d}\times \reals^n$, $\algprivols(X, Y) = w_{OLS} + \tau$, with $w = (X^\top X)^{-1}X^\top Y$ and $\tau$ is a random noise variable. Assume $Y\leq R$, then $w_{OLS}\leq \frac{\lambda_{\max}(X^\top X)R}{\lambda_{\min}(X^\top X)}$. 

\begin{corollary}
    [Pre-processing robust DP guarantees of $\algprivols$]
    Let $\cP_\alpha$ be a set of projection matrices of size $d\times k$ and bounded inverse operator norm, \ie $\forall P_1, P_2\in \cP_\alpha$, $P_1, P_2 \in \reals^{d\times k}$ and $\norm{P_1^{-\top} P_1^{-1} - P_2^{-\top} P_2^{-1}}\leq \alpha$. Define the set of pre-processing matrices $\Pi_{\cP_L} = \{\pi(X, Y) = (XP, Y): P\in \cP_L\}$. Then, if $\algprivols$ is $(\epsilon, 0)$-DP for any $\pi\in \Pi_{\cP_L}$, it is $\br{\epsilon', 0}$-DP for $\Pi_{\cP_L}$ with \[\epsilon' = \br{1 + \frac{\alpha R}{\zeta}}\epsilon,\] where $\zeta = \max_{w_1(S_1), w_2(S_2): S_1\Delta S_2 - 1} \norm{w_1 - w_2}_2$, $w(S) \leq R, \forall S$. 
\end{corollary}


\begin{proof}
    For $\algprivols$ to be $(\epsilon, 0)$-DP with respect to any $\pi\in \Pi_{\cP_L}$, it suffices to sample $\tau$ from Laplacian distribution with scale parameter $\frac{\sqrt{n}\zeta}{\lambda_{\min}\epsilon}$ because the sensitivity of $\algprivols \circ \pi$ is bounded by \[\zeta_1 \leq \max_{P \in \cP_\alpha}\max_{w_1, w_2}\norm{P^{-1} w_1 - P^{-1} w_2}_1 \leq \max_{P \in \cP_\alpha}\max_{w_1, w_2}\sqrt{n}\norm{ w_1 -  w_2}_2 \norm{P^{-\top}P^{-1}}\leq  \frac{\sqrt{n}\zeta}{\lambda_{\min}},\] where $\zeta = \max_{w_1, w_2}\norm{w_1 - w_2}_2$ and $\lambda_{\min} = \min_{P\in \cP} \lambda_{\min}(P^\top P)$. 

    To achieve pre-processing robust DP with respect to $\Pi_{\cP_L}$, we calculate the sensitivity over the maximum of pre-processing functions $\pi_1, \pi_2\in \Pi_{\cP_L}$, 
    \begin{equation}
    \begin{aligned}
            \zeta_2 &= \max_{\pi_1, \pi_2\in \Pi_{\cP_L}} \max_{S_1, S_2: S_1\Delta S_2 = 1} \norm{\cA\circ\pi_1(S_1) - \cA\circ\pi_2(S_1) }_1 \\
            &\leq \sqrt{n} \max_{\pi_1, \pi_2\in \Pi_{\cP_L}} \max_{S_1, S_2: S_1\Delta S_2 = 1} \norm{\cA\circ\pi_1(S_1) - \cA\circ\pi_2(S_1) }_2 \\
            &=\max_{P_1, P_2\in \cP_\alpha}\max_{w_1, w_2}\sqrt{n} \norm{\Lambda_1 w_1 - \Lambda_2 w_2}_2 \\
            &= \max_{P_1, P_2\in \cP_\alpha}\max_{w_1, w_2}\sqrt{n} \norm{\Lambda_1 w_1 - \Lambda_1 w_2 + \Lambda_1 w_2 - \Lambda_2 w_2}_2\\
            &\leq \max_{P_1, P_2\in \cP_\alpha}\max_{w_1, w_2}\sqrt{n}\br{\sqrt{\norm{\Lambda_1w_1 - \Lambda_1 w_2}_2^2 + \norm{(\Lambda_1 - \Lambda_2)w_2}_2^2 - 2(w_1 - w_2)^\top \Lambda_1^\top (\Lambda_1 - \Lambda_2)w_2}}\\
            &\leq\sqrt{n\br{\max_{w_1, w_2, P_1, P_2\in \cP_\alpha}\norm{\Lambda_1w_1 - \Lambda_1 w_2}_2^2 + \max_{w_1, w_2, P_1, P_2\in \cP_\alpha}\norm{(\Lambda_1 - \Lambda_2)w_2}_2^2 - 2(w_1 - w_2)^\top \Lambda_1^\top (\Lambda_1 - \Lambda_2)w_2}}\\
            &\leq \sqrt{n\br{\zeta_1^2 + \alpha^2 R^2 + 2\zeta_1\alpha R}} = \sqrt{n}\br{\zeta_1 + \alpha R}
    \end{aligned}
    \end{equation}
    where $\Lambda_1 = P_1^{-1}$ and $\Lambda_2 = P_2^{-1}$ and $w_1, w_2$ denote the OLS estimators of $S_1, S_2$ respectively, and $R$ is the upper bound on $w$. 

    Solving \[\frac{\zeta_1}{\epsilon} = \frac{\zeta_2}{\epsilon'},\]
    we have \[\epsilon' = \br{1 + \frac{\alpha R}{\zeta}}\epsilon. \]
\end{proof}
% \begin{corollary}[Privacy upper bound of $\algprivols$ for two pre-processing functions]
%     There exists $D_1, D_2\in \reals^{d\times k}$ corresponding to two pre-processing functions $\pi_i(X, Y) = (X D_i, Y)$ for $i\in \{1, 2\}$, such that if private low-dimensional OLS $\algprivols$ is $(\epsilon, 0)$-DP with respect to the space pre-processed by $\pi_1$ and $\pi_2$, then $\algprivols$ is $(\epsilon', 0)$-pre-processing robust DP for $\Pi = \{\pi_1, \pi_2\}$, where $\epsilon' = f(\algprivols, \Pi, \epsilon)$. 
% \end{corollary}


Conjecture: $D_1, D_2$ satisfies some properties: eg. RIP with respect to the data space (both projections lead to good accuracy), then $\epsilon'\approx \epsilon$. Without any constraint, we can choose $D_1, D_2$ s.t. $\epsilon' \ll \epsilon$, but the algorithm with projection $D_2$ cannot achieve a relatively high accuracy. 

\paragraph{Private low dimensional OLS estimators}
Let $w_1, w_2$ be the OLS estimators from two neighboring datasets $S_1 = (X_1, Y_1), S_2 = (X_2, Y_2)$ differing only at the point $(x, y)$. For a projection matrix $D\in \reals^{d\times k}$ that transforms the original datasets to $(X_1D, Y), (X_2D, Y)$, simple algebra shows that the low-dimensional OLS estimators are $D^{-1}w_1, D^{-1}w_2$ respectively. Here, we use $D^{-1}$ to denote the Moore-Penrose inverse of $D$. Then, we define the private OLS estimators in the projected space as $\what_1 = D^{-1}w_1 + n_1$, $\what_2 = D^{-1} w_2 + n_2$, where $n_1, n_2\sim \cN(0, \sigma^2I_k)$. Denote the PDF of $\what_1, \what_2$ by $f_1, f_2$, then, 

\begin{equation}
    \begin{aligned}
        f_1(x) &= \frac{1}{(2\pi)^{1/d}\sigma}\exp\br{-\frac{\norm{x - D^{-1}w_1}^2_2}{2\sigma^2}}\\
        f_2(x) &= \frac{1}{(2\pi)^{1/d}\sigma}\exp\br{-\frac{\norm{x - D^{-1}w_2}^2_2}{2\sigma^2}}
    \end{aligned}
\end{equation}

Then,
\begin{equation}
    \begin{aligned}
        \log \frac{f_1(x)}{f_2(x)} &= \frac{1}{2\sigma^2}\br{\norm{x-D^{-1}w_2}^2_2 - \norm{x-D^{-1}w_1}^2_2} \\
        &= \frac{1}{2\sigma^2}\br{2\br{w_1 - w_2}^\top D^{-\top} x + w_2^\top D^{-\top} D^{-1}w_2 - w_1^\top D^{-\top} D^{-1}w_1}\\
        &= \frac{1}{2\sigma^2}\br{2\br{w_1 - w_2}^\top D^{-\top} x + w_2^\top \Sigma_Dw_2 - w_1^\top \Sigma_Dw_1}, 
    \end{aligned}
\end{equation}
where $\Sigma_D = D^{-\top} D^{-1}$. 

For the estimator $\what$ to be $(\epsilon, \delta)$-DP, 
\begin{equation}
    \bP_{x\sim f_1}\br{\log \frac{f_1(x)}{f_2(x)}\geq \epsilon}\leq \delta 
\end{equation}
\begin{equation}
    \begin{aligned}
        \bP_{x\sim f_1}\bs{\log \frac{f_1(x)}{f_2(x)}\geq \epsilon} &= \bP_{x\sim f_1}\bs{\frac{1}{2\sigma^2}\br{2\br{w_1 - w_2}^\top D^{-\top} x + w_2^\top \Sigma_Dw_2 - w_1^\top \Sigma_Dw_1}\geq \epsilon }\\
        &= \bP_{x\sim f_1}\bs{\br{w_1 - w_2}^\top D^{-\top}x\geq \sigma^2 \epsilon + \frac{w_1^\top \Sigma_D w_1}{2}-\frac{w_2^\top \Sigma_D w_2}{2}}\\
        &= \bP_{Z \sim \cN(0, 1)}\bs{ Z\geq \frac{\sigma^2 \epsilon + \frac{1}{2}\br{w_1 - w_2}^\top \Sigma_D \br{w_1 + w_2} - (w_1-w_2)^\top \Sigma_D w_1}{\sqrt{\sigma^2 (w_1 - w_2)^\top \Sigma_D (w_1 - w_2)}}}\\
        &= \bP_{Z\sim \cN(0, 1)}\bs{Z\geq \frac{2\sigma^2 \epsilon - (w_1 - w_2)^\top \Sigma_D (w_1 - w_2)}{2\sigma \sqrt{(w_1-w_2)^\top \Sigma_D (w_1 - w_2)}}}\\
        &= \bP_{Z\sim \cN(0, 1)} \bs{Z \geq \frac{\sigma\epsilon}{\norm{w_1-w_2}_{\Sigma_D}} - \frac{\norm{w_1 - w_2}_{\Sigma_D}}{2\sigma}} \\
        & \leq \delta, 
    \end{aligned}
\end{equation}
where $\norm{v}^2_{\Sigma_D} = v^\top\Sigma_D v$ for any vector $v\sim \reals^d$, and the last inequality follows by \[\sigma \geq \frac{\norm{w_1 - w_2}_{\Sigma_D}\sqrt{2\log \frac{1}{\delta} }+ \norm{w_1 - w_2}_{\Sigma_D}^2}{\epsilon}.\] 
Let the $\ell_2$-sensitivity of the non-private low-dimensional OLS estimators be $\zeta$, then setting $\sigma = \frac{\zeta}{\epsilon}\br{\sqrt{2\log\frac{1}{\delta}} + \zeta}$ ensures $(\epsilon, \delta)$-DP of the private low-dimensional OLS. 

\begin{equation}
    \bP_{x\sim f_1}\bs{\max_{w_1, w_2:\text{from neighboring dataset}} \log \frac{f_1(x)}{f_2(x)}\geq \epsilon}
\end{equation}

\paragraph{Different fixed projection matrices $D_1, D_2$}
For two projection matrices $D_1, D_2\in \reals^{d\times k}$, we project two neighboring datasets $S_1$, $S_2$ into the low dimensional space with $D_1, D_2$ respectively, $\Stilde_1 = (X_1 D_1, Y_1)$, $\Stilde_2 = (X_2D_2, Y_2)$. Thus, the OLS estimators in the projected spaces are $D_1^{-1}\what_1$ and $D_2^{-1}\what_2$. Let the private OLS estimator in the projected spaces be $\wtilde_1 = D_1^{-1}\what_1 + n_1$ and $\wtilde_2 = D_2^{-1}\what_1 + n_2$ for $n_1, n_2\sim \cN(0, \sigma^2)$. Let $\ftilde_1, \ftilde_2$ be the PDF of $\wtilde_1, \wtilde_2$, then 
\begin{equation}
    \begin{aligned}
        \ftilde_1(x) &= \frac{1}{(2\pi)^{1/d}\sigma}\exp\br{-\frac{\norm{x - D_1^{-1}w_1}^2_2}{2\sigma^2}}\\
        \ftilde_2(x) &= \frac{1}{(2\pi)^{1/d}\sigma}\exp\br{-\frac{\norm{x - D_2^{-1}w_2}^2_2}{2\sigma^2}}
    \end{aligned}
\end{equation}
Then, 
\begin{equation}
    \begin{aligned}
        \log \frac{\ftilde_1(x)}{\ftilde_2(x)} &= \frac{1}{2\sigma^2}\br{\norm{x-D_2^{-1}w_2}^2_2 - \norm{x-D_1^{-1}w_1}^2_2} \\
        &= \frac{1}{2\sigma^2}\br{2\br{w_1^\top D^{-\top}_1 - w_2^\top D^{-\top}_2}  x + w_2^\top D^{-\top}_2 D^{-1}_2w_2 - w_1^\top D^{-\top}_1 D^{-1}_1w_1}\\
        &= \frac{1}{2\sigma^2}\br{2\br{w_1^\top D^{-\top}_1 - w_2^\top D^{-\top}_2} x + w_2^\top \Sigma_2w_2 - w_1^\top \Sigma_1w_1}, 
    \end{aligned}
\end{equation}
where $\Sigma_1 = D^{-\top}_1D^{-1}_1$ and $\Sigma_2 = D^{-\top}_2D^{-1}_2$. 

Then, for $x$ sampled from $\ftilde_1$, \begin{equation}
    \begin{aligned}
        \bP_{x\sim \ftilde_1}\bs{\log\frac{\ftilde_1(x)}{\ftilde_2(x)}\geq \epsilon'} &= \bP_{x\sim \ftilde_1}\bs{\br{w_1^\top D_1^{-\top} - w_2^\top D_2^{-\top}}x\geq \epsilon'\sigma^2 - \frac{w_2^\top \Sigma_2 w_2}{2} + \frac{w_1^\top \Sigma_1 w_1}{2}}\\
        &= \bP_{Z\sim \cN(0, 1)}\bs{Z\geq \frac{\epsilon'\sigma^2 + \frac{w_1^\top \Sigma_1 w_1}{2} - \frac{w_2^\top \Sigma_2 w_2}{2} - \br{D_1^{-1}w_1 - D_2^{-1}w_2}^\top D_1^{-1}w_1}{\sqrt{\sigma^2 \br{D_1^{-1}w_1 - D_2^{-1}w_2}^\top\br{D_1^{-1}w_1 - D_2^{-1}w_2}}}}\\
        &= \bP_{Z\sim \cN(0, 1)}\bs{Z\geq \frac{\epsilon'\sigma^2 - \frac{w_1^\top \Sigma_1 w_1}{2} - \frac{w_2^\top \Sigma_2 w_2}{2}  +w_2^\top \Sigma_{21}w_1}{\sigma \sqrt{w_1^\top \Sigma_1 w_1 + w_2^\top \Sigma_2 w_2 - 2w_2^\top \Sigma_{21}w_1}}}\\
        &= \bP_{Z\sim \cN(0, 1)}\bs{Z\geq \frac{\epsilon \sigma}{\sqrt{A}} + \frac{\sqrt{A}}{2\sigma}}
    \end{aligned}
\end{equation} 
where $\Sigma_{21y} = D_2^{-\top} D_1^{-1}$ and $A = w_1^\top \Sigma_1 w_1 +w_2^\top \Sigma_2 w_2 - 2w_2^\top \Sigma_{21} w_1 $.  

For the same $\delta$ and choose $D_1 = D$, we require \begin{equation}
    \epsilon' = \frac{\sqrt{A}\epsilon}{\norm{w_1 - w_2}_{\Sigma_1}} + \frac{\sqrt{A}\br{\sqrt{A} - \norm{w_1 - w_2}_{\Sigma_1}}}{2\sigma^2},
\end{equation}

Choose $\Lambda_1$ such that $\Lambda_1 w_2 = 0$. Choose $\Lambda_2$ such that its largest eigenvector is of the same direction as $w_2$ and $\Lambda_2^\top \Lambda_1 = 0$. 

Then, choose the eigenvalues of $\Lambda_2$ such that $w_2\top (\Lambda_2^\top \Lambda_2)w_2 \leq 2w_1^\top (\Lambda_1^\top \Lambda_1)w_1$. Then, we have $\epsilon' \leq \epsilon$. 

For $\Lambda_2\prec \Lambda_1$, then \begin{equation}
    \begin{aligned}
        A &= 
    \end{aligned}
\end{equation}

For fixed $D_1 = \Lambda_1^{-1}$, finding $D_2$ that maximizes $\epsilon'$ is equivalent to finding $\Lambda_2 = D_2^{-1}$ that maximizes $\sqrt{A}$, \ie 
\begin{equation}\label{eq:optimization-lambda}
    \begin{aligned}
        \Lambda_2 &= \text{arg}\max_{\Lambda_2:\norm{\Lambda_2^{-1}x} \geq (1-\eta)\norm{x}}\sqrt{A} \\
        &= \text{arg}\max_{\Lambda_2:\norm{\Lambda_2^{-1}x} \geq (1-\eta)\norm{x} } w_1^\top \Sigma_1 w_1 + w_2^\top \Sigma_2 w_2 - 2w_2^\top \Sigma_{21}w_1\\
        & = \text{arg}\max_{\Lambda_2:\norm{\Lambda_2^{-1}x} \geq (1-\eta)\norm{x}}  w_2^\top \Lambda_2^\top \Lambda_2 w_2 - 2w_2^\top \Lambda_2^\top \Lambda_1 w_1\\
        &= \text{arg}\max_{\Lambda_2:\norm{\Lambda_2^{-1}x} \geq (1-\eta)\norm{x}} w_2^\top \Lambda_2^\top \br{\Lambda_2 w_2 - \Lambda_1 w_1} =: \text{arg}\max_{\Lambda_2}g
    \end{aligned}
\end{equation}
The function $g$ is convex with respect to each entry of $\Lambda_2^{ij}$, $i\in [k], j\in [d]$. As the function is smooth, solving the optimization with PSGD leads to asymptotic maximum. 

% Assume that the instance space $\cX$ is compact and convex. Denote the set of extreme points as $\cE$. Using Carathéodory's theorem, $\Lambda$ is $\eta$-RIP on all points in $\cX$ is implied by the following constraints, for any pair of extreme points $x_1, x_2\in \cE$,
% \begin{equation}
%     \br{\Lambda x_1}^\top \Lambda x_2 \geq \br{1-\eta} x_1^\top x_2 
% \end{equation}
% and for any point $x\in \cE$, 
% \begin{equation}
%     \br{\Lambda x}^\top \Lambda x \geq \br{1-\eta}\norm{x}_2. 
% \end{equation}
Let the instance space $\cX$ be the $\cX = \{x\in \bR^d: \norm{x}_2 = 1\}$, and let $b_i = (0, \ldots, 1, \ldots, 0)$ be the vector that is $1$ at the $ith$ entry and $0$ elsewhere. Then, any point $x\in \cX$ can be expressed as a weighted sum of $b_i's$, $i\in [d]$, \ie 
\begin{equation}
    x = \sum_{i = 1}^d x_i b_i
\end{equation}
Note that for any $x\in \cX$, $\sum_{i = 1}^dx_i^2 = 1$ by the definition of $\cX$. Then, for any $x\in \cX$, 
\begin{equation}
    \begin{aligned}
        \norm{D^\top x}_2^2 = \norm{D^\top \br{\sum_{i = 1}^d x_i b_i}}^2_2 = \norm{\sum_{i = 1}^d x_i Db_i}^2_2 = \sum_{i, j = 1}^d x_i x_j D_j^\top D_i 
    \end{aligned}
\end{equation}
where $D_j\in \reals^k$ represents the $jth$ row of the matrix $D\in \reals^{d\times k}$. 

As $\norm{x_i} = 1$, \begin{equation}
  \sum_{i, j = 1}^d D_j^\top D_i  \leq \norm{D^\top x}_2^2 \leq d \sum_{i, j = 1}^d D_j^\top D_i
\end{equation}

As 
\begin{equation}
    1 = \norm{x^\top x} = \norm{x^\top D^{-\top} D^\top x}\leq \norm{x^\top D^{-\top}}\norm{D^\top x} = \norm{\Lambda x} \norm{D^\top x},
\end{equation} 
combine it with RIP condition of the projection matrix $1+\eta \geq \norm{D^\top x}\geq 1-\eta$, we can write \begin{equation}\label{eq:opt-constraint1}
    d\sum_{i, j = 1}^d \Lambda_j^\top \Lambda_i \geq \norm{\Lambda x}\geq \frac{1}{\norm{D^\top x}}\geq \frac{1}{1+\eta}
\end{equation}
where $\Lambda_j\in \reals^k$ represents the $jth$ column of the matrix $\Lambda = D^{-1} \in \reals^{k\times d}$. 

With the constraint in~\Cref{eq:opt-constraint1}, the attacker should choose $\Lambda_2$ as the solution of a constrained concave optimization problem. We can write the Lagrangian form of the problem as
\begin{equation}
    \cL(\lambda, \Lambda_2) = w_2^\top \Lambda_2^\top  (\Lambda_2 w_2 -\Lambda_1w_1) + \lambda \br{\frac{1}{d(1+\eta)} - \sum_{i, j = 1}^d \Lambda_j^\top \Lambda_i}
\end{equation}

\begin{equation}
\begin{aligned}
       \frac{ \partial g}{\partial \Lambda_2^{ij}} &= \frac{\partial \sum_{j = 1}^k\br{\sum_{i = 1}^d w_2^i \Lambda_2^{ji}}^2 - \sum_{j = 1}^k \br{\sum_{i = 1}^d w_2^i \Lambda_2^{ji}}\br{\sum_{i= 1}^d 2_1^i \Lambda_1^{ij}}}{\partial \Lambda_2^{ji}}\\
       &= \frac{\partial}{\partial\Lambda_2^{ij}}\br{\sum_{j = 1}^k \sum_{i, \ell = 1}^d w_2^i w_2^\ell \Lambda_2^{ji} \Lambda_2^{j\ell}  - \sum_{j = 1}^k \sum_{i, \ell = 1}^d w_2^i w_1^\ell \Lambda_2^{ji} \Lambda_1^{j\ell} }\\
       &=  2\sum_{\ell =1 }^d w_2^\ell w_2^j \Lambda_2^{i\ell}- \sum_{\ell =1 }^d w_1^\ell w_2^j \Lambda_1^{i\ell}
       \\
       &= \br{2\Lambda_2^{(i)} w_2 -\Lambda_1^{(i)}w_1}w_2^j = 0
\end{aligned}
\end{equation}
where $\Lambda_1^{(i)}$ denotes the $i$th row of the matrix $\Lambda_1$. 

Second derivative 
\begin{equation}
    \begin{aligned}
        \frac{\partial g}{\partial \Lambda_2^{ij}} &= \br{w_2^i}^2 \geq 0
    \end{aligned}
\end{equation}

Assume the $(X_1, Y_1) = \{(X_2, Y_2)\cup (x, y)\}$, then we can express the relationship between $w_1$ and $w_2$, 
\begin{equation}\label{eq:relationship-w1-w2-deriv}
\begin{aligned}
        w_1 &= \br{X_2^\top X_2 + x x^\top}^{-1}\br{X_2^\top Y + x^\top y}\\
        &= \br{(X_2^\top X_2)^{-1} + (X_2^\top X_2)^{-1}(xx^\top)\br{X_2^\top X_2 + x x^\top}^{-1}} \br{X_2^\top Y + x^\top y}\\
        &= w_2 + \br{X_2^\top X_2}^{-1} (xx^\top)w_1 + \br{X_2^\top X_2}^{-1}x^\top y 
\end{aligned}
\end{equation}
Rearranging~\Cref{eq:relationship-w1-w2-deriv}, we have 
\begin{equation}\label{eq:relationship-w1-w2}
    w_1 = \br{I_d - \br{X_2^\top X_2}^{-1} xx^\top}^{-1}w_2 + \br{I_d - \br{X_2^\top X_2}^{-1} xx^\top}^{-1} (X_2^\top X_2)^{-1}x^T y
\end{equation}

Substituting~\Cref{eq:relationship-w1-w2} into~\Cref{eq:optimization-lambda}, we can write the optimization problem as \begin{equation}
    \label{eq:optimization-lambda2}
    \begin{aligned}
        \Lambda_2 &= \text{arg}\max_{\Lambda_2:\norm{\Lambda_2x}\geq (1-\eta)\norm{x}} w_2^\top \Lambda_2^\top \Lambda_2\br{I_d - \Sigma_X^{-1}xx^\top }^{-1} w_2 - w_2^\top \Lambda_2^\top \Lambda_1 \br{\Sigma_X - xx^\top}^{-1} x^\top y\\
        &= \text{arg}\max_{\Lambda_2:\norm{\Lambda_2x}\geq (1-\eta)\norm{x}} Y^\top X \Sigma_X^{-1} \Lambda_2^\top \Lambda_2 \br{\Sigma_X - xx^\top}^{-1} X^\top Y - Y^\top X \Sigma_X^{-1} \Lambda_2^\top \Lambda_1 \br{\Sigma_X - xx^\top}^{-1} x^\top y\\
        &= \text{arg}\max_{\Lambda_2:\norm{\Lambda_2x}\geq (1-\eta)\norm{x}} Y^\top X \Sigma_X^{-1} \Lambda_2^\top \br{\Lambda_2 \br{\Sigma_X - xx^\top}^{-1} X^\top Y - \Lambda_1 \br{\Sigma_X - xx^\top}^{-1}  x^\top y}
    \end{aligned}
\end{equation}


